Fast and Small Subsampled R-indexes

The $r$-index represented a breakthrough in compressed indexing of repetitive text collections, outperforming its alternatives by orders of magnitude in query time. Its space usage, $O(r)$ where $r$ is the number of runs in the Burrows--Wheeler Transform of the text, is however higher than Lempel--Ziv (LZ) and grammar-based indexes, and makes it uninteresting in various real-life scenarios of milder repetitiveness. We introduce the $sr$-index, a variant that limits the space to $O(\min(r,n/s))$ for a text of length $n$ and a given parameter $s$, at the expense of multiplying by $s$ the time per occurrence reported. The $sr$-index is obtained subsampling the text positions indexed by the $r$-index, being still able to support pattern matching with guaranteed performance. Our experiments show that the theoretical analysis falls short in describing the practical advantages of the $sr$-index, because it performs much better on real texts than on synthetic ones: the $sr$-index retains the performance of the $r$-index while using 1.5--4.0 times less space, sharply outperforming {\em virtually every other} compressed index on repetitive texts in both time and space. Only a particular LZ-based index uses less space than the $sr$-index, but it is an order of magnitude slower. Our second contribution are the $r$-csa and $sr$-csa indexes. Just like the $r$-index adapts the well-known FM-Index to repetitive texts, the $r$-csa adapts Sadakane's Compressed Suffix Array (CSA) to this case. We show that the principles used on the $r$-index turn out to fit naturally and efficiently in the CSA framework. The $sr$-csa is the corresponding subsampled version of the $r$-csa. While the CSA performs better than the FM-Index on classic texts with alphabets larger than DNA, we show that the $sr$-csa outperforms the $sr$-index on repetitive texts over those larger alphabets and some DNA texts as well.

==> alg/alg-rcsa-count-toehold.tex <==
\begin{algorithm}[t]
  \IO{Query pattern $\vPat[1..\vsPat]$.}
  {Range $\langle \vsp,\vep \rangle$ on $\SA$ for $\vPat$;
  Value $\SA[\vsp]$.}

  \begin{multicols}{2}
    \subimport{./}{fn-rcsa-count-toehold}
  \end{multicols}
  \BlankLine

  \caption{Counting pattern occurrences and finding value $\SA[\vsp]$ with $\RCSA$.}
  \label{alg:rcsa_count_toehold}
\end{algorithm}

==> alg/fn-rcsa-count-toehold.tex <==
\SetKwFunction{fnCount}{count}
\SetKwFunction{fnToehold}{findToehold}

\Function{\fnCount{$\vPat[1..\vsPat]$}}{
  $\langle \vsp, \vep \rangle \leftarrow \langle 1, \vsTColl \rangle$\;
  $v \leftarrow n$\;

  \For{$i \leftarrow \vsPat$ \KwDownTo $1$}{
    $c \leftarrow \vPat[i]$\;

    $v \leftarrow \fnToehold(v, \vsp, c)$\;

    $\vsp \leftarrow C[c] + \rank_{c}(\Psi, \vsp-1) + 1$\;
    $\vep \leftarrow C[c] + \rank_{c}(\Psi, \vep)$\;
    \If{$\vsp > \vep$} {\Return{``$\vPat$ is not in $\vTColl$''}}
  }

  \Return{$\langle \langle \vsp, \vep \rangle, v \rangle$}\;
}
\BlankLine
\BlankLine

\Function{\fnToehold{$v$, $\vsp$, $c$}}{\label{fn:NextSPAndToehold}
  $\langle k, f_{\Psi}, l_{\Psi} \rangle \leftarrow \findRun(\Psi, \vsp, c)$\;
  \If{$f_{\Psi} \le \vsp < l_{\Psi}$}{\Return{$v - 1$}}
  \Return{$\SamplesF[k]$}\;
}

==> img/base-bwt.tex <==
\begin{scope}[name prefix = BWT-]
  \node[name=name, CellHeader]{$\mathit{BWT}$};
  \node[name=0, right=0cm of name, Cell, Block] {a};
  \node[name=1, right=0cm of 0, Cell, Block] {d};
  \node[name=2, right=0cm of 1, Cell, BlockStart] {l};
  \node[name=3, right=0cm of 2, Cell, BlockMid] {l};
  \node[name=4, right=0cm of 3, Cell, BlockEnd] {l};
  \node[name=5, right=0cm of 4, Cell, Block] {r};
  \node[name=6, right=0cm of 5, Cell, Block] {\$};
  \node[name=7, right=0cm of 6, Cell, Block] {a};
  \node[name=8, right=0cm of 7, Cell, BlockStart] {b};
  \node[name=9, right=0cm of 8, Cell, BlockEnd] {b};
  \node[name=10, right=0cm of 9, Cell, BlockStart] {a};
  \node[name=11, right=0cm of 10, Cell, BlockEnd] {a};
  \node[name=12, right=0cm of 11, Cell, Block] {r};
  \node[name=13, right=0cm of 12, Cell, BlockStart] {a};
  \node[name=14, right=0cm of 13, Cell, BlockMid] {a};
  \node[name=15, right=0cm of 14, Cell, BlockMid] {a};
  \node[name=16, right=0cm of 15, Cell, BlockMid] {a};
  \node[name=17, right=0cm of 16, Cell, BlockEnd] {a};
\end{scope}


==> img/base-i-psi.tex <==
\begin{scope}[name prefix = Psi-i-]
  \node[name=name, CellHeader]{$I_{\Psi}$};
  \node[name=0, right=0cm of name, Cell] {1};
  \node[name=1, right=0cm of 0, Cell] {2};
  \node[name=2, right=0cm of 1, Cell] {3};
  \node[name=3, right=0cm of 2, Cell] {4};
  \node[name=4, right=0cm of 3, Cell] {};
  \node[name=5, right=0cm of 4, Cell] {6};
  \node[name=6, right=0cm of 5, Cell] {};
  \node[name=7, right=0cm of 6, Cell] {};
  \node[name=8, right=0cm of 7, Cell] {};
  \node[name=9, right=0cm of 8, Cell] {};
  \node[name=10, right=0cm of 9, Cell] {11};
  \node[name=11, right=0cm of 10, Cell] {};
  \node[name=12, right=0cm of 11, Cell] {13};
  \node[name=13, right=0cm of 12, Cell] {14};
  \node[name=14, right=0cm of 13, Cell] {};
  \node[name=15, right=0cm of 14, Cell] {};
  \node[name=16, right=0cm of 15, Cell] {17};
  \node[name=17, right=0cm of 16, Cell] {18};
\end{scope}


==> img/base-pos.tex <==
\begin{scope}[name prefix = Pos-]
  \node[CellHeader](name) {$\#$};
  \foreach \x [remember=\x as \lastx (initially name)] in {1, ..., 18}
  \node[right=0cm of \lastx, Cell](\x) {\x};
\end{scope}


==> img/base-psi.tex <==
\begin{scope}[name prefix = Psi-]
  \node[name=name, CellHeader]{$\Psi$};
  \node[name=0, right=0cm of name, Cell, Block] {7};
  \node[name=1, right=0cm of 0, Cell, Block] {1};
  \node[name=2, right=0cm of 1, Cell, Block] {8};
  \node[name=3, right=0cm of 2, Cell, BlockStart] {11};
  \node[name=4, right=0cm of 3, Cell, BlockEnd] {12};
  \node[name=5, right=0cm of 4, Cell, BlockStart] {14};
  \node[name=6, right=0cm of 5, Cell, BlockMid] {15};
  \node[name=7, right=0cm of 6, Cell, BlockMid] {16};
  \node[name=8, right=0cm of 7, Cell, BlockMid] {17};
  \node[name=9, right=0cm of 8, Cell, BlockEnd] {18};
  \node[name=10, right=0cm of 9, Cell, BlockStart] {9};
  \node[name=11, right=0cm of 10, Cell, BlockEnd] {10};
  \node[name=12, right=0cm of 11, Cell, Block] {2};
  \node[name=13, right=0cm of 12, Cell, BlockStart] {3};
  \node[name=14, right=0cm of 13, Cell, BlockMid] {4};
  \node[name=15, right=0cm of 14, Cell, BlockEnd] {5};
  \node[name=16, right=0cm of 15, Cell, Block] {6};
  \node[name=17, right=0cm of 16, Cell, Block] {13};
\end{scope}


==> img/base-sa.tex <==
\begin{scope}[name prefix = SA-]
  \node[CellHeader](name) {$\mathit{SA}$};
  \node[right=0cm of name, Cell, Block](0) {18};
  \node[right=0cm of 0, Cell, BlockStart](1) {17};
  \node[right=0cm of 1, Cell, BlockMid](2) {9};
  \node[right=0cm of 2, Cell, BlockMid](3) {3};
  \node[right=0cm of 3, Cell, BlockMid](4) {12};
  \node[right=0cm of 4, Cell, BlockMid](5) {7};
  \node[right=0cm of 5, Cell, BlockMid](6) {1};
  \node[right=0cm of 6, Cell, BlockMid](7) {10};
  \node[right=0cm of 7, Cell, BlockMid](8) {5};
  \node[right=0cm of 8, Cell, BlockEnd](9) {14};
  \node[right=0cm of 9, Cell, BlockStart](10) {4};
  \node[right=0cm of 10, Cell, BlockEnd](11) {13};
  \node[right=0cm of 11, Cell, Block](12) {16};
  \node[right=0cm of 12, Cell, BlockStart](13) {8};
  \node[right=0cm of 13, Cell, BlockMid](14) {2};
  \node[right=0cm of 14, Cell, BlockEnd](15) {11};
  \node[right=0cm of 15, Cell, BlockStart](16) {6};
  \node[right=0cm of 16, Cell, BlockEnd](17) {15};
\end{scope}


==> img/base-text.tex <==
\begin{scope}[name prefix = T-]
  \node[name=name, CellHeader]{$\mathcal{T}$};
  \node[name=0, right=0cm of name, Cell] {a};
  \node[name=1, right=0cm of 0, Cell] {l};
  \node[name=2, right=0cm of 1, Cell] {a};
  \node[name=3, right=0cm of 2, Cell] {b};
  \node[name=4, right=0cm of 3, Cell] {a};
  \node[name=5, right=0cm of 4, Cell] {r};
  \node[name=6, right=0cm of 5, Cell] {a};
  \node[name=7, right=0cm of 6, Cell] {l};
  \node[name=8, right=0cm of 7, Cell] {a};
  \node[name=9, right=0cm of 8, Cell] {a};
  \node[name=10, right=0cm of 9, Cell] {l};
  \node[name=11, right=0cm of 10, Cell] {a};
  \node[name=12, right=0cm of 11, Cell] {b};
  \node[name=13, right=0cm of 12, Cell] {a};
  \node[name=14, right=0cm of 13, Cell] {r};
  \node[name=15, right=0cm of 14, Cell] {d};
  \node[name=16, right=0cm of 15, Cell] {a};
  \node[name=17, right=0cm of 16, Cell] {\$};
\end{scope}


==> img/experiments/r-csa/dna-real.tex <==
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.45\textwidth]{img/experiments/r-csa/dr-Chr19-locate}
    \includegraphics[width=0.45\textwidth]{img/experiments/r-csa/dr-Salmonella-locate}

    \includegraphics[width=0.80\textwidth]{img/experiments/r-csa/dna-real-legend}
  \end{center}
  \caption{Space-time tradeoffs for the real DNA collections.}
  \label{fig:rcsa-dna-real}
\end{figure}


==> img/experiments/r-csa/dna-synthetic.tex <==
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.45\textwidth]{img/experiments/r-csa/ds-DNA-001-locate}
    \includegraphics[width=0.45\textwidth]{img/experiments/r-csa/ds-DNA-003-locate}
    \includegraphics[width=0.45\textwidth]{img/experiments/r-csa/ds-DNA-010-locate}
    \includegraphics[width=0.45\textwidth]{img/experiments/r-csa/ds-DNA-030-locate}

    \includegraphics[width=0.80\textwidth]{img/experiments/r-csa/dna-synthetic-legend}
  \end{center}
  \caption{Space-time tradeoffs for the synthetic DNA collections.}
  \label{fig:rcsa-dna-synthetic}
\end{figure}


==> img/experiments/r-csa/pizzachilli-documents.tex <==
\begin{figure}[t]
  \begin{center}
%    \includegraphics[width=0.49\textwidth]{img/experiments/r-csa/influenza-locate}
%    \includegraphics[width=0.49\textwidth]{img/experiments/r-csa/cere-locate}
%    \includegraphics[width=0.49\textwidth]{img/experiments/r-csa/para-locate}
%    \includegraphics[width=0.49\textwidth]{img/experiments/r-csa/escherichia-locate}
    \includegraphics[width=0.45\textwidth]{img/experiments/r-csa/pc-einstein-locate}
    \includegraphics[width=0.45\textwidth]{img/experiments/r-csa/pc-kernel-locate}
    \includegraphics[width=0.45\textwidth]{img/experiments/r-csa/pc-worldleaders-locate}
    \includegraphics[width=0.45\textwidth]{img/experiments/r-csa/pc-coreutils-locate}

    \includegraphics[width=0.90\textwidth]{img/experiments/r-csa/pizzachilli-documents-legend}
  \end{center}
  \caption{Space-time tradeoffs for the PizzaChili document collections.}
  \label{fig:rcsa-pizzachilli-documents}
\end{figure}


==> img/experiments/r-csa/pizzachilli-genomes.tex <==
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.45\textwidth]{img/experiments/r-csa/pc-influenza-locate}
    \includegraphics[width=0.45\textwidth]{img/experiments/r-csa/pc-cere-locate}
    \includegraphics[width=0.45\textwidth]{img/experiments/r-csa/pc-para-locate}
    \includegraphics[width=0.45\textwidth]{img/experiments/r-csa/pc-escherichia-locate}
%    \includegraphics[width=0.49\textwidth]{img/experiments/r-csa/einstein-locate}
%    \includegraphics[width=0.49\textwidth]{img/experiments/r-csa/kernel-locate}
%    \includegraphics[width=0.49\textwidth]{img/experiments/r-csa/worldleaders-locate}
%    \includegraphics[width=0.49\textwidth]{img/experiments/r-csa/coreutils-locate}

    \includegraphics[width=0.90\textwidth]{img/experiments/r-csa/pizzachilli-genomes-legend}
  \end{center}
  \caption{Space-time tradeoffs for the PizzaChili genomes collections.}
  \label{fig:rcsa-pizzachilli-genomes}
\end{figure}


==> img/extra/dna-synthetic/ds-sampling-densities-fig.tex <==
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.90\textwidth]{img/extra/dna-synthetic/marks-densities-kde-0.25-DNA-001}
%    \includegraphics[width=0.45\textwidth]{img/extra/dna-synthetic/marks-densities-kde-0.25-DNA-003}
%    \includegraphics[width=0.45\textwidth]{img/extra/dna-synthetic/marks-densities-kde-0.25-DNA-010}
    \includegraphics[width=0.90\textwidth]{img/extra/dna-synthetic/marks-densities-kde-0.25-DNA-030}
  \end{center}
  \caption{
    Distribution of original and subsampled $\BWT$-run heads within the synthetic DNA datasets.
    The $x$-axis represents the positions of these run heads along the text.
    The $y$-axis shows the density, which indicates how frequently $\BWT$-run heads appear at different locations.
    The smooth curve is obtained using the statistical method Kernel Density Estimation (KDE).
  }
  \label{fig:ds-sampling-densities}
\end{figure}


==> img/extra/ds-marks-densities-fig.tex <==
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.90\textwidth]{img/extra/marks-densities-kde-0.25}
  \end{center}
  \caption{
    Distribution of $\BWT$-run heads within the Pizza-Chili text datasets.
    The $x$-axis represents the positions of these run heads along the text.
    The $y$-axis shows the density, which indicates how frequently $\BWT$-run heads appear at different locations.
    The smooth curve is obtained using the statistical method Kernel Density Estimation (KDE).
  }
  \label{fig:samples-densities}
\end{figure}


==> img/extra/ds-samples-densities-fig.tex <==
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.90\textwidth]{img/extra/ds-marks-densities-kde-0.25}
    \includegraphics[width=0.90\textwidth]{img/extra/ds-marks-densities-hist-0.25}
  \end{center}
  \caption{
    Distribution of $\BWT$-run heads within the synthetic DNA datasets.
    The $x$-axis represents the positions of these run heads along the text.
    The $y$-axis shows the density, which indicates how frequently $\BWT$-run heads appear at different locations.
    The smooth curve is obtained using the statistical method Kernel Density Estimation (KDE).
  }
  \label{fig:ds-samples-densities}
\end{figure}


==> img/extra/pizza-chili/pc-dna-sampling-densities-fig.tex <==
\begin{figure}[t]
  \begin{center}
%    \includegraphics[width=0.90\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-einstein}
%    \includegraphics[width=0.45\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-kernel}
%    \includegraphics[width=0.45\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-world_leaders}
    \includegraphics[width=0.90\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-influenza}
%    \includegraphics[width=0.90\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-coreutils}
    \includegraphics[width=0.90\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-cere}
    \includegraphics[width=0.45\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-para}
    \includegraphics[width=0.45\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-escherichia}
  \end{center}
  \caption{
    Distribution of original and subsampled $\BWT$-run heads within the Pizza-Chili repetitive texts \cite{PizzaChili}.
    The $x$-axis represents the positions of these run heads along the text.
    The $y$-axis shows the density, which indicates how frequently $\BWT$-run heads appear at different locations.
    The smooth curve is obtained using the statistical method Kernel Density Estimation (KDE).
  }
  \label{fig:pc-dna-sampling-densities}
\end{figure}


==> img/extra/pizza-chili/pc-doc-sampling-densities-fig.tex <==
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.90\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-einstein}
    \includegraphics[width=0.45\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-kernel}
    \includegraphics[width=0.45\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-world_leaders}
%    \includegraphics[width=0.90\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-influenza}
    \includegraphics[width=0.90\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-coreutils}
%    \includegraphics[width=0.90\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-cere}
%    \includegraphics[width=0.45\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-para}
%    \includegraphics[width=0.45\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-escherichia}
  \end{center}
  \caption{
    Distribution of original and subsampled $\BWT$-run heads within the Pizza-Chili repetitive texts \cite{PizzaChili}.
    The $x$-axis represents the positions of these run heads along the text.
    The $y$-axis shows the density, which indicates how frequently $\BWT$-run heads appear at different locations.
    The smooth curve is obtained using the statistical method Kernel Density Estimation (KDE).
  }
  \label{fig:pc-doc-sampling-densities}
\end{figure}


==> img/extra/pizza-chili/pc-sampling-densities-fig.tex <==
\begin{figure}[t]
  \begin{center}
    \includegraphics[width=0.90\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-einstein}
%    \includegraphics[width=0.45\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-kernel}
%    \includegraphics[width=0.45\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-world_leaders}
%    \includegraphics[width=0.90\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-influenza}
%    \includegraphics[width=0.90\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-coreutils}
    \includegraphics[width=0.90\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-cere}
%    \includegraphics[width=0.90\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-para}
    \includegraphics[width=0.90\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-escherichia}
  \end{center}
  \caption{
    Distribution of original and subsampled $\BWT$-run heads within the Pizza-Chili repetitive texts \cite{PizzaChili}.
    The $x$-axis represents the positions of these run heads along the text.
    The $y$-axis shows the density, which indicates how frequently $\BWT$-run heads appear at different locations.
    The smooth curve is obtained using the statistical method Kernel Density Estimation (KDE).
  }
  \label{fig:pc-sampling-densities}
\end{figure}


==> img/extra/sampling-densities-fig.tex <==
\begin{figure}[tp]
  \begin{center}
    \includegraphics[width=0.85\textwidth]{img/extra/dna-synthetic/marks-densities-kde-0.25-DNA-001}
%    \includegraphics[width=0.45\textwidth]{img/extra/dna-synthetic/marks-densities-kde-0.25-DNA-003}
%    \includegraphics[width=0.45\textwidth]{img/extra/dna-synthetic/marks-densities-kde-0.25-DNA-010}
    \includegraphics[width=0.85\textwidth]{img/extra/dna-synthetic/marks-densities-kde-0.25-DNA-030}
    \includegraphics[width=0.85\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-einstein}
%    \includegraphics[width=0.45\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-kernel}
%    \includegraphics[width=0.45\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-world_leaders}
%    \includegraphics[width=0.90\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-influenza}
%    \includegraphics[width=0.90\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-coreutils}
    \includegraphics[width=0.85\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-cere}
%    \includegraphics[width=0.90\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-para}
    \includegraphics[width=0.85\textwidth]{img/extra/pizza-chili/marks-densities-kde-0.25-escherichia}
  \end{center}
  \caption{
    Distribution of original and subsampled $\BWT$-run heads within the synthetic DNA datasets and Pizza-Chili repetitive texts.
    The $x$-axis represents the positions of these run heads along the text. The $y$-axis shows the density, which indicates how frequently $\BWT$-run heads appear at different locations. The original distributions are shown with the lightest color, and darker colors are used for subsampling with larger values of $s$.
    The smooth curve is obtained using Kernel Density Estimation (KDE).
  }
  \label{fig:sampling-densities}
\end{figure}


==> img/extra/sampling-frequencies-zoom-fig.tex <==
\begin{figure}[tp]
  \begin{center}
    \includegraphics[width=0.90\textwidth]{img/extra/dna-synthetic/marks-densities-freq-DNA-001}
%    \includegraphics[width=0.45\textwidth]{img/extra/dna-synthetic/marks-densities-freq-DNA-003}
%    \includegraphics[width=0.45\textwidth]{img/extra/dna-synthetic/marks-densities-freq-DNA-010}
    \includegraphics[width=0.90\textwidth]{img/extra/dna-synthetic/marks-densities-freq-DNA-030}
%    \includegraphics[width=0.85\textwidth]{img/extra/pizza-chili/marks-densities-freq-einstein}
%    \includegraphics[width=0.45\textwidth]{img/extra/pizza-chili/marks-densities-freq-kernel}
%    \includegraphics[width=0.45\textwidth]{img/extra/pizza-chili/marks-densities-freq-world_leaders}
%    \includegraphics[width=0.90\textwidth]{img/extra/pizza-chili/marks-densities-freq-influenza}
%    \includegraphics[width=0.90\textwidth]{img/extra/pizza-chili/marks-densities-freq-coreutils}
%    \includegraphics[width=0.85\textwidth]{img/extra/pizza-chili/marks-densities-freq-cere}
%    \includegraphics[width=0.90\textwidth]{img/extra/pizza-chili/marks-densities-freq-para}
%    \includegraphics[width=0.95\textwidth]{img/extra/pizza-chili/marks-densities-freq-escherichia}
    \includegraphics[width=0.45\textwidth]{img/extra/pizza-chili/zoom/marks-densities-freq-cere-part-3}
    \hspace{3pt}
    \includegraphics[width=0.45\textwidth]{img/extra/pizza-chili/zoom/marks-densities-freq-escherichia-part-1}
%    \includegraphics[width=0.45\textwidth]{img/extra/pizza-chili/zoom/marks-densities-freq-para-part-3}
  \end{center}
  \caption{
    Distribution of original and subsampled $\BWT$-run heads within the synthetic DNA datasets and Pizza-Chili repetitive texts.
    The $x$-axis represents the positions of these run heads along the text. The $y$-axis indicates how frequently $\BWT$-run heads appear at different locations. The original distributions are shown with the lightest color, and darker colors are used for subsampling with larger values of $s$.
  }
  \label{fig:sampling-frequencies}
\end{figure}


==> img/rcsa-counting-psi.tex <==
\begin{scope}[name prefix = Psi-]
  \node[name=name, CellHeader]{$\Psi$};
  \node[name=0, right=0cm of name, Cell, Block, Highlight1] {7};
  \node[name=1, right=0cm of 0, Cell, Block, Highlight1] {1};
  \node[name=2, right=0cm of 1, Cell, Block, Highlight1] {8};
  \node[name=3, right=0cm of 2, Cell, BlockStart, Highlight1] {11};
  \node[name=4, right=0cm of 3, Cell, BlockEnd] {12};
  \node[name=5, right=0cm of 4, Cell, BlockStart, Highlight1] {14};
  \node[name=6, right=0cm of 5, Cell, BlockMid] {15};
  \node[name=7, right=0cm of 6, Cell, BlockMid] {16};
  \node[name=8, right=0cm of 7, Cell, BlockMid] {17};
  \node[name=9, right=0cm of 8, Cell, BlockEnd] {18};
  \node[name=10, right=0cm of 9, Cell, BlockStart, Highlight1] {9};
  \node[name=11, right=0cm of 10, Cell, BlockEnd] {10};
  \node[name=12, right=0cm of 11, Cell, Block, Highlight1] {2};
  \node[name=13, right=0cm of 12, Cell, BlockStart, Highlight1] {3};
  \node[name=14, right=0cm of 13, Cell, BlockMid] {4};
  \node[name=15, right=0cm of 14, Cell, BlockEnd] {5};
  \node[name=16, right=0cm of 15, Cell, Block, Highlight1] {6};
  \node[name=17, right=0cm of 16, Cell, Block, Highlight1] {13};
\end{scope}

\begin{scope}[decoration={brace,raise=1.3ex},black!65]
  \draw [decorate] (Psi-0.north west) to node [above=1.5ex] {$\Psi_{\text{\$}}$} (Psi-0.north east);
  \draw [decorate] (Psi-1.north west) to node [above=1.5ex] {$\Psi_{\text{a}}$} (Psi-9.north east);
  \draw [decorate] (Psi-10.north west) to node [above=1.5ex] {$\Psi_{\text{b}}$} (Psi-11.north east);
  \draw [decorate] (Psi-12.north west) to node [above=1.5ex] {$\Psi_{\text{d}}$} (Psi-12.north east);
  \draw [decorate] (Psi-13.north west) to node [above=1.5ex] {$\Psi_{\text{l}}$} (Psi-15.north east);
  \draw [decorate] (Psi-16.north west) to node [above=1.5ex] {$\Psi_{\text{r}}$} (Psi-17.north east);
\end{scope}


==> img/rcsa-phi-1-bwt.tex <==
\begin{scope}[name prefix = BWT-]
  \node[name=name, CellHeader]{$\mathit{BWT}$};
  \node[name=0, right=0cm of name, Cell, Block] {a};
  \node[name=1, right=0cm of 0, Cell, Block] {d};
  \node[name=2, right=0cm of 1, Cell, BlockStart] {l};
  \node[name=3, right=0cm of 2, Cell, BlockMid, label={[label distance=-2pt]below:$i$}] {l};
  \node[name=4, right=0cm of 3, Cell, BlockEnd] {l};
  \node[name=5, right=0cm of 4, Cell, Block, Highlight3, label={[label distance=-2pt]below:$l$}] {r};
  \node[name=6, right=0cm of 5, Cell, Block] {\$};
  \node[name=7, right=0cm of 6, Cell, Block] {a};
%  \node[name=8, right=0cm of 7, Cell, BlockStart, Highlight1, label={[label distance=-2pt]below:j}] {b};
  \node[name=8, right=0cm of 7, Cell, BlockStart, Highlight1] {b};
  \node[name=9, right=0cm of 8, Cell, BlockEnd, Highlight2] {b};
%  \node[name=10, right=0cm of 9, Cell, BlockStart, label={[label distance=-2pt]below:i}] {a};
  \node[name=10, right=0cm of 9, Cell, BlockStart, Highlight1, label={[label distance=-2pt]below:$j$}] {a};
  \node[name=11, right=0cm of 10, Cell, BlockEnd, Highlight2] {a};
  \node[name=12, right=0cm of 11, Cell, Block, Highlight4, label={[label distance=-2pt]below:$f$}] {r};
  \node[name=13, right=0cm of 12, Cell, BlockStart] {a};
  \node[name=14, right=0cm of 13, Cell, BlockMid] {a};
  \node[name=15, right=0cm of 14, Cell, BlockMid] {a};
  \node[name=16, right=0cm of 15, Cell, BlockMid, Highlight1] {a};
  \node[name=17, right=0cm of 16, Cell, BlockEnd, Highlight2] {a};
\end{scope}

%\draw[Arrow] (BWT-8.north) to [bend left=20] node[near start,above=-2pt,sloped,font=\small] {$\Psi^1(j)$} (BWT-16.north);
%\draw[ArrowDash] (BWT-9.north) to [bend left=20] (BWT-17.north);
%\draw[Arrow] (BWT-16.south) to [bend left=15] node[near start,below=-2pt,sloped,font=\small] {$\Psi^2(j)$} (BWT-5.south);
%\draw[ArrowDash] (BWT-17.south) to [bend left=25] (BWT-12.south);

\draw[Arrow] (BWT-10.north) to [bend right=45] node[midway,above=-2pt,font=\small] {$\Psi^1(j)$} (BWT-8.north);
\draw[ArrowDash] (BWT-11.north) to [bend right=45] (BWT-9.north);
\draw[Arrow] (BWT-8.south) to [bend right=20] node[midway,below=-2pt,font=\small] {$\Psi^2(j)$} (BWT-16.south);
\draw[ArrowDash] (BWT-9.south) to [bend right=20] (BWT-17.south);
\draw[Arrow] (BWT-16.north) to [bend right=20] node[midway,above=-2pt,font=\small] {$\Psi^{\Delta}(j)$} (BWT-5.north);
\draw[ArrowDash] (BWT-17.north) to [bend right=35] (BWT-12.north);

\draw[ArrowDot] (BWT-5.south) to [bend right=25] (BWT-12.south);


==> img/rcsa-phi-1-draft.tex <==
%! Author = Dustin Cobas <dustin.cobas@gmail.com>
%! Date = 8/12/2023

\begin{figure}[t]
    \begin{center}
        \includestandalone[width=1\textwidth]{./pos}
    \end{center}
    \begin{center}
        \includestandalone[width=1\textwidth]{./rcsa-scheme-text}
    \end{center}
    \begin{center}
        \includestandalone[width=1\textwidth]{./rcsa-phi-1-mark}
    \end{center}
%    \begin{center}
%        \includestandalone[width=1\textwidth]{./rcsa-phi-1-sa-old}
%    \end{center}
    \begin{center}
        \includestandalone[width=1\textwidth]{./rcsa-scheme-sa}
    \end{center}
%    \begin{center}
%        \includestandalone[width=1\textwidth]{./psi}
%    \end{center}
%    \begin{center}
%        \includestandalone[width=1\textwidth]{./psi-diff}
%    \end{center}
    \begin{center}
        \includestandalone[width=1\textwidth]{./rcsa-phi-1-bwt}
    \end{center}
    \begin{center}
        \includestandalone[width=1\textwidth]{./bwt}
    \end{center}
    \begin{center}
        \includestandalone[width=1\textwidth]{./bwt-pos}
    \end{center}
    \caption{Schematic example of the sampling mechanism of the $\RCSA$.
    There is a run border between $j_3-1$ and $j_3$.}
    \label{fig:scheme-rcsa-draft}
\end{figure}


==> img/rcsa-phi-1-psi.tex <==
\begin{scope}[name prefix = Psi-]
  \node[name=name, CellHeader]{$\Psi$};
  \node[name=0, right=0cm of name, Cell, Block] {7};
  \node[name=1, right=0cm of 0, Cell, Block] {1};
  \node[name=2, right=0cm of 1, Cell, Block] {8};
  \node[name=3, right=0cm of 2, Cell, BlockStart, Highlight1, label={[label distance=-2pt]below:$i$}] {11};
  \node[name=4, right=0cm of 3, Cell, BlockEnd, Highlight2, label={[label distance=-2pt]below:$i+1$}] {12};
  \node[name=5, right=0cm of 4, Cell, BlockStart] {14};
  \node[name=6, right=0cm of 5, Cell, BlockMid] {15};
  \node[name=7, right=0cm of 6, Cell, BlockMid] {16};
  \node[name=8, right=0cm of 7, Cell, BlockMid, Highlight1] {17};
  \node[name=9, right=0cm of 8, Cell, BlockEnd, Highlight2] {18};
  \node[name=10, right=0cm of 9, Cell, BlockStart, Highlight1] {9};
  \node[name=11, right=0cm of 10, Cell, BlockEnd, Highlight2] {10};
  \node[name=12, right=0cm of 11, Cell, Block] {2};
  \node[name=13, right=0cm of 12, Cell, BlockStart] {3};
  \node[name=14, right=0cm of 13, Cell, BlockMid] {4};
  \node[name=15, right=0cm of 14, Cell, BlockEnd] {5};
  \node[name=16, right=0cm of 15, Cell, Block, Highlight3, label={[label distance=-2pt]below:$l$}] {6};
  \node[name=17, right=0cm of 16, Cell, Block, Highlight4, label={[label distance=-2pt]below:$l+1$}] {13};
\end{scope}

% Step arrows
\draw[Arrow] (Psi-3.north) to [bend left=30] node[midway,above=-2pt,font=\small] {$\Psi^1(i)$} (Psi-10.north);
\draw[ArrowDash] (Psi-4.north) to [bend left=30] (Psi-11.north);
\draw[Arrow] (Psi-10.south) to [bend left=45] node[midway,below=-2pt,font=\small] {$\Psi^2(i)$} (Psi-8.south);
\draw[ArrowDash] (Psi-11.south) to [bend left=45] (Psi-9.south);
\draw[Arrow] (Psi-8.north) to [bend left=25] node[midway,above=-2pt,font=\small] {$\Psi^{\Delta}(i)$} (Psi-16.north);
\draw[ArrowDash] (Psi-9.north) to [bend left=25] (Psi-17.north);

%\draw[ArrowDot] (Psi-16.south) to [bend right=45] (Psi-17.south);


==> img/rcsa-phi-1-sa.tex <==
\begin{scope}[name prefix = SA-]
  \node[CellHeader](name) {$\mathit{SA}$};
  \node[right=0cm of name, Cell, Block](0) {18};
  \node[right=0cm of 0, Cell, BlockStart](1) {17};
  \node[right=0cm of 1, Cell, BlockMid](2) {9};
  \node[right=0cm of 2, Cell, BlockMid, Highlight1](3) {3};
  \node[right=0cm of 3, Cell, BlockMid, Highlight2](4) {12};
  \node[right=0cm of 4, Cell, BlockMid](5) {7};
  \node[right=0cm of 5, Cell, BlockMid](6) {1};
  \node[right=0cm of 6, Cell, BlockMid](7) {10};
  \node[right=0cm of 7, Cell, BlockMid, Highlight1](8) {5};
  \node[right=0cm of 8, Cell, BlockEnd, Highlight2](9) {14};
  \node[right=0cm of 9, Cell, BlockStart, Highlight1](10) {4};
  \node[right=0cm of 10, Cell, BlockEnd, Highlight2](11) {13};
  \node[right=0cm of 11, Cell, Block](12) {16};
  \node[right=0cm of 12, Cell, BlockStart](13) {8};
  \node[right=0cm of 13, Cell, BlockMid](14) {2};
  \node[right=0cm of 14, Cell, BlockEnd](15) {11};
  \node[right=0cm of 15, Cell, BlockStart, Highlight3](16) {6};
  \node[right=0cm of 16, Cell, BlockEnd, Highlight4](17) {15};
\end{scope}


==> img/rcsa-phi-1-text.tex <==
\begin{scope}[name prefix = T-]
  \node[name=name, CellHeader]{$\mathcal{T}$};
  \node[name=0, right=0cm of name, Cell] {a};
  \node[name=1, right=0cm of 0, Cell] {l};
  \node[name=2, right=0cm of 1, Cell, Highlight1, label={[label distance=-2pt,font=\scriptsize]below:$\SA[i]$}] {a};
  \node[name=3, right=0cm of 2, Cell, Highlight1] {b};
  \node[name=4, right=0cm of 3, Cell, Highlight1] {a};
  \node[name=5, right=0cm of 4, Cell, Highlight3, label={[label distance=-2pt,font=\scriptsize]below:$\SA[l]$}] {r};
  \node[name=6, right=0cm of 5, Cell] {a};
  \node[name=7, right=0cm of 6, Cell] {l};
  \node[name=8, right=0cm of 7, Cell] {a};
  \node[name=9, right=0cm of 8, Cell] {a};
  \node[name=10, right=0cm of 9, Cell] {l};
  \node[name=11, right=0cm of 10, Cell, Highlight2, label={[label distance=-2pt,font=\scriptsize]below:$\SA[i+1]$}] {a};
  \node[name=12, right=0cm of 11, Cell, Highlight2] {b};
  \node[name=13, right=0cm of 12, Cell, Highlight2] {a};
  \node[name=14, right=0cm of 13, Cell, Highlight4, label={[label distance=-2pt,font=\scriptsize]below:$\SA[l+1]$}] {r};
  \node[name=15, right=0cm of 14, Cell] {d};
  \node[name=16, right=0cm of 15, Cell] {a};
  \node[name=17, right=0cm of 16, Cell] {\$};
\end{scope}

%\draw[Arrow] (T-2.south) to [bend right=30] node[midway,below=-2pt,font=\small] {$\Delta=3$} (T-5.south);
%\draw[ArrowDash] (T-11.south) to [bend right=30] node[midway,below=-2pt,font=\small] {$\Delta=3$} (T-14.south);

\draw[Arrow] (T-2.north) to [bend left=30] node[midway,above=-2pt,font=\small] {$\Delta$} (T-5.north);
\draw[ArrowDash] (T-11.north) to [bend left=30] node[midway,above=-2pt,font=\small] {$\Delta$} (T-14.north);


==> img/rcsa-scheme-sa.tex <==
\begin{scope}[name prefix = SA-]
  \node[CellHeader](name) {$\mathit{SA}$};
  \node[right=0cm of name, Cell, Block, Highlight1](0) {18};
  \node[right=0cm of 0, Cell, BlockStart, Highlight1](1) {17};
  \node[right=0cm of 1, Cell, BlockMid, Highlight1](2) {9};
  \node[right=0cm of 2, Cell, BlockMid, Highlight1](3) {3};
  \node[right=0cm of 3, Cell, BlockMid](4) {12};
  \node[right=0cm of 4, Cell, BlockMid, Highlight1](5) {7};
  \node[right=0cm of 5, Cell, BlockMid](6) {1};
  \node[right=0cm of 6, Cell, BlockMid](7) {10};
  \node[right=0cm of 7, Cell, BlockMid](8) {5};
  \node[right=0cm of 8, Cell, BlockEnd](9) {14};
  \node[right=0cm of 9, Cell, BlockStart, Highlight1](10) {4};
  \node[right=0cm of 10, Cell, BlockEnd](11) {13};
  \node[right=0cm of 11, Cell, Block, Highlight1](12) {16};
  \node[right=0cm of 12, Cell, BlockStart, Highlight1](13) {8};
  \node[right=0cm of 13, Cell, BlockMid](14) {2};
  \node[right=0cm of 14, Cell, BlockEnd](15) {11};
  \node[right=0cm of 15, Cell, BlockStart, Highlight1](16) {6};
  \node[right=0cm of 16, Cell, BlockEnd, Highlight1](17) {15};
\end{scope}


==> img/rcsa-scheme-text-head.tex <==
\begin{scope}[name prefix = T-]
  \node[name=name, CellHeader]{$\mathcal{T}$};
  \node[name=0, right=0cm of name, Cell] {a};
  \node[name=1, right=0cm of 0, Cell] {l};
  \node[name=2, right=0cm of 1, Cell, Highlight1] {a};
  \node[name=3, right=0cm of 2, Cell, Highlight1] {b};
  \node[name=4, right=0cm of 3, Cell] {a};
  \node[name=5, right=0cm of 4, Cell, Highlight1] {r};
  \node[name=6, right=0cm of 5, Cell, Highlight1] {a};
  \node[name=7, right=0cm of 6, Cell, Highlight1] {l};
  \node[name=8, right=0cm of 7, Cell, Highlight1] {a};
  \node[name=9, right=0cm of 8, Cell] {a};
  \node[name=10, right=0cm of 9, Cell] {l};
  \node[name=11, right=0cm of 10, Cell] {a};
  \node[name=12, right=0cm of 11, Cell] {b};
  \node[name=13, right=0cm of 12, Cell] {a};
  \node[name=14, right=0cm of 13, Cell, Highlight1] {r};
  \node[name=15, right=0cm of 14, Cell, Highlight1] {d};
  \node[name=16, right=0cm of 15, Cell, Highlight1] {a};
  \node[name=17, right=0cm of 16, Cell, Highlight1] {\$};
\end{scope}


==> img/rcsa-scheme-text.tex <==
\begin{scope}[name prefix = T-]
  \node[name=name, CellHeader]{$\mathcal{T}$};
  \node[name=0, right=0cm of name, Cell] {a};
  \node[name=1, right=0cm of 0, Cell] {l};
  \node[name=2, right=0cm of 1, Cell] {a};
  \node[name=3, right=0cm of 2, Cell] {b};
  \node[name=4, right=0cm of 3, Cell] {a};
  \node[name=5, right=0cm of 4, Cell, Highlight1] {r};
  \node[name=6, right=0cm of 5, Cell] {a};
  \node[name=7, right=0cm of 6, Cell] {l};
  \node[name=8, right=0cm of 7, Cell, Highlight1] {a};
  \node[name=9, right=0cm of 8, Cell] {a};
  \node[name=10, right=0cm of 9, Cell, Highlight1] {l};
  \node[name=11, right=0cm of 10, Cell, Highlight1] {a};
  \node[name=12, right=0cm of 11, Cell, Highlight1] {b};
  \node[name=13, right=0cm of 12, Cell, Highlight1] {a};
  \node[name=14, right=0cm of 13, Cell, Highlight1] {r};
  \node[name=15, right=0cm of 14, Cell, Highlight1] {d};
  \node[name=16, right=0cm of 15, Cell, Highlight1] {a};
  \node[name=17, right=0cm of 16, Cell, Highlight1] {\$};
\end{scope}


==> img/srcsa-scheme-sa-del.tex <==
\tikzstyle{Crossed} = [cross out, black!50, line width = .1em]

\begin{scope}[name prefix = SA-Del-]
%  \node[CellHeader](name) {$\mathit{SA}$};
%  \node[right=0cm of name, Cell, Block, Highlight1](0) {18};
  \node[right=0cm of SA-0, Cell, Crossed](1) {}; %{17};
%  \node[right=0cm of 1, Cell, BlockMid, Highlight1](2) {9};
%  \node[right=0cm of SA-2, Cell, BlockMid, Crossed](3) {3};
%  \node[right=0cm of 3, Cell, BlockMid](4) {12};
  \node[right=0cm of SA-4, Cell, Crossed](5) {}; %{7};
%  \node[right=0cm of 5, Cell, BlockMid](6) {1};
%  \node[right=0cm of 6, Cell, BlockMid](7) {10};
%  \node[right=0cm of 7, Cell, BlockMid](8) {5};
%  \node[right=0cm of 8, Cell, BlockEnd](9) {14};
  \node[right=0cm of SA-9, Cell, Crossed](10) {}; %{4};
%  \node[right=0cm of 10, Cell, BlockEnd](11) {13};
  \node[right=0cm of SA-11, Cell, Crossed](12) {}; %{16};
  \node[right=0cm of SA-12, Cell, Crossed](13) {}; %{8};
%  \node[right=0cm of 13, Cell, BlockMid](14) {2};
%  \node[right=0cm of 14, Cell, BlockEnd](15) {11};
%  \node[right=0cm of SA-15, Cell, Crossed](16) {}; %{6};
%  \node[right=0cm of 16, Cell, BlockEnd, Highlight1](17) {15};
\end{scope}


==> img/srcsa-scheme-sa.tex <==
\begin{scope}[name prefix = SA-]
  \node[CellHeader](name) {$\mathit{SA}$};
  \node[right=0cm of name, Cell, Block, Highlight1](0) {18};
  \node[right=0cm of 0, Cell, BlockStart](1) {17};
  \node[right=0cm of 1, Cell, BlockMid, Highlight1](2) {9};
  \node[right=0cm of 2, Cell, BlockMid, Highlight1](3) {3};
  \node[right=0cm of 3, Cell, BlockMid](4) {12};
  \node[right=0cm of 4, Cell, BlockMid](5) {7};
  \node[right=0cm of 5, Cell, BlockMid](6) {1};
  \node[right=0cm of 6, Cell, BlockMid](7) {10};
  \node[right=0cm of 7, Cell, BlockMid](8) {5};
  \node[right=0cm of 8, Cell, BlockEnd](9) {14};
  \node[right=0cm of 9, Cell, BlockStart](10) {4};
  \node[right=0cm of 10, Cell, BlockEnd](11) {13};
  \node[right=0cm of 11, Cell, Block](12) {16};
  \node[right=0cm of 12, Cell, BlockStart](13) {8};
  \node[right=0cm of 13, Cell, BlockMid](14) {2};
  \node[right=0cm of 14, Cell, BlockEnd](15) {11};
  \node[right=0cm of 15, Cell, BlockStart, Highlight1](16) {6};
  \node[right=0cm of 16, Cell, BlockEnd, Highlight1](17) {15};
\end{scope}


==> img/srcsa-scheme-text.tex <==
\begin{scope}[name prefix = T-]
  \node[name=name, CellHeader]{$\mathcal{T}$};
  \node[name=0, right=0cm of name, Cell] {a};
  \node[name=1, right=0cm of 0, Cell] {l};
  \node[name=2, right=0cm of 1, Cell] {a};
  \node[name=3, right=0cm of 2, Cell] {b};
  \node[name=4, right=0cm of 3, Cell] {a};
  \node[name=5, right=0cm of 4, Cell, Highlight1] {r};
  \node[name=6, right=0cm of 5, Cell] {a};
  \node[name=7, right=0cm of 6, Cell] {l};
  \node[name=8, right=0cm of 7, Cell, Highlight1] {a};
  \node[name=9, right=0cm of 8, Cell] {a};
  \node[name=10, right=0cm of 9, Cell, Highlight1] {l};
  \node[name=11, right=0cm of 10, Cell] {a};
  \node[name=12, right=0cm of 11, Cell] {b};
  \node[name=13, right=0cm of 12, Cell] {a};
  \node[name=14, right=0cm of 13, Cell, Highlight1] {r};
  \node[name=15, right=0cm of 14, Cell] {d};
  \node[name=16, right=0cm of 15, Cell, Highlight1] {a};
  \node[name=17, right=0cm of 16, Cell] {\$};
\end{scope}


==> img/tikz_styles.tex <==
%! Author = Dustin Cobas <dustin.cobas@gmail.com>
%! Date = 8/13/2023

%% Fill Color Styles
\tikzstyle{Highlight1} = [fill=gray!35]
\tikzstyle{Highlight2} = [fill=gray!35, densely dashed]
\tikzstyle{Highlight3} = [fill=black!60]
\tikzstyle{Highlight4} = [fill=black!60, densely dashed]

%% Element Styles
\tikzstyle{CellHeaderBase} = [font=\ttfamily \bfseries \normalsize, minimum width=5em]
\tikzstyle{CellBase} = [draw=black!75, font=\ttfamily \bfseries \small, minimum width=\linewidth/20, minimum height=3.5ex, inner sep=1pt]

\tikzstyle{Block} = [chamfered rectangle, chamfered rectangle angle=35]
\tikzstyle{BlockStart} = [Block, chamfered rectangle corners={north west, south west}]
\tikzstyle{BlockMid} = [Block, chamfered rectangle corners=none]
\tikzstyle{BlockEnd} = [Block, chamfered rectangle corners={north east, south east}]

\tikzstyle{Arrow} = [-Stealth, black!75, thick]
\tikzstyle{ArrowDash} = [-Stealth, densely dashed, black!55, thick]
\tikzstyle{ArrowDot} = [-Stealth, densely dotted, black!75, thick]

